On the relaxation of Gauss's capillarity theory under spanning conditions

We study a variational model for soap films in which the films are represented by sets with fixed small volume rather than surfaces. In this problem, a minimizing sequence of completely "wet" films, or sets of finite perimeter spanning a wire frame, may converge to a film containing both wet regions of positive volume and collapsed (dry) surfaces. When collapsing occurs, these limiting objects lie outside the original minimization class and instead are admissible for a relaxed problem. Here we show that the relaxation and the original formulation are equivalent by approximating the collapsed films in the relaxed class by wet films in the original class.

==> references.tex <==
@article {ACV,
    AUTHOR = {Ambrosio, Luigi and Colesanti, Andrea and Villa, Elena},
     TITLE = {Outer {M}inkowski content for some classes of closed sets},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {342},
      YEAR = {2008},
    NUMBER = {4},
     PAGES = {727--748},
      ISSN = {0025-5831},
   MRCLASS = {28A75 (49Q15)},
  MRNUMBER = {2443761},
MRREVIEWER = {Daniel Hug},
       DOI = {10.1007/s00208-008-0254-z},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/s00208-008-0254-z},
}

@article {HP16b,
    AUTHOR = {Harrison, J. and Pugh, H.},
     TITLE = {Solutions to the {R}eifenberg {P}lateau problem with
              cohomological spanning conditions},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {55},
      YEAR = {2016},
    NUMBER = {4},
     PAGES = {Art. 87, 37},
      ISSN = {0944-2669,1432-0835},
   MRCLASS = {49Q05 (49J45 49Q10 49Q20 55N05)},
  MRNUMBER = {3519161},
MRREVIEWER = {Jan\ Mal\'{y}},
       DOI = {10.1007/s00526-016-1022-7},
       URL = {https://doi.org/10.1007/s00526-016-1022-7},
}

@article{foamdrainageII,
title = {Foam drainage on the microscale {II}. Imaging flow through single Plateau borders},
journal = {Journal of Colloid and Interface Science},
volume = {276},
number = {2},
pages = {439-449},
year = {2004},
issn = {0021-9797},
doi = {https://doi.org/10.1016/j.jcis.2003.12.060},
url = {https://www.sciencedirect.com/science/article/pii/S0021979704000475},
author = {S.A. Koehler and S. Hilgenfeldt and E.R. Weeks and H.A. Stone},
keywords = {Foams, Emulsions, Surface rheology},
abstract = {The liquid in foam forms an interconnected network, which is composed of Plateau borders, nodes, and films. One of the dominant pathways for foam drainage is flow through Plateau borders, and we use confocal microscopy to obtain experimental results for the flow fields inside individual Plateau borders. For three types of surfactants detailed comparisons are made with a model based upon the influence of surface viscosity at free boundaries between the gas in the bubbles and the liquid in the Plateau borders. The model describes the flows well, and we find good agreement between the surface viscosity predicted by this model and representative values found in the literature. We also give a qualitative description of the flow in the nodes.}
}

@article{foamdrainageI,
title = {Foam drainage on the microscale: I. Modeling flow through single Plateau borders},
journal = {Journal of Colloid and Interface Science},
volume = {276},
number = {2},
pages = {420-438},
year = {2004},
issn = {0021-9797},
doi = {https://doi.org/10.1016/j.jcis.2003.12.061},
url = {https://www.sciencedirect.com/science/article/pii/S0021979704000487},
author = {S.A. Koehler and S. Hilgenfeldt and H.A. Stone},
keywords = {Foams, Emulsions, Surface rheology},
abstract = {The drainage of liquid through a foam involves flow in channels, also called Plateau borders, which generally are long and slender. We model this flow by assuming the flow is unidirectional, the shear is transverse to the flow direction, and the liquid/gas interfaces are mobile and characterized by a Newtonian surface viscosity, which does not depend on the shear rate. Numerical finite difference simulations are performed, and analytical approximations for the velocity fields inside the channels and the films that separate the bubbles are given. We compare the liquid flow rates through interior channels, exterior channels (i.e., channels contacting container walls) and films. We find that when the number of exterior channels is comparable to the number of interior channels, i.e., narrow container geometries, the exterior channels can significantly affect the dynamics of the drainage process. Even for highly mobile interfaces, the films do not significantly contribute to the drainage process, unless the amount of liquid in the films is within a factor of ten of the amount of liquid in the channels.}
}

@book {AFP,
    AUTHOR = {Ambrosio, Luigi and Fusco, Nicola and Pallara, Diego},
     TITLE = {Functions of bounded variation and free discontinuity
              problems},
    SERIES = {Oxford Mathematical Monographs},
 PUBLISHER = {The Clarendon Press, Oxford University Press, New York},
      YEAR = {2000},
     PAGES = {xviii+434},
      ISBN = {0-19-850245-1},
   MRCLASS = {49-02 (49J45 49K10 49Qxx)},
  MRNUMBER = {1857292},
MRREVIEWER = {J. E. Brothers},
}

@article {BP,
    AUTHOR = {B\'{e}rard, Pierre and Meyer, Daniel},
     TITLE = {In\'{e}galit\'{e}s isop\'{e}rim\'{e}triques et applications},
   JOURNAL = {Ann. Sci. \'{E}cole Norm. Sup. (4)},
  FJOURNAL = {Annales Scientifiques de l'\'{E}cole Normale Sup\'{e}rieure. Quatri\`eme
              S\'{e}rie},
    VOLUME = {15},
      YEAR = {1982},
    NUMBER = {3},
     PAGES = {513--541},
      ISSN = {0012-9593},
   MRCLASS = {58G25 (35P15 52A40 53C20 58G30)},
  MRNUMBER = {690651},
MRREVIEWER = {J. Peetre},
       URL = {http://www.numdam.org/item?id=ASENS_1982_4_15_3_513_0},
}

@article{Brakke05,
title = {Instability of the wet cube cone soap film},
journal = {Colloids and Surfaces A: Physicochemical and Engineering Aspects},
volume = {263},
number = {1},
pages = {4-10},
year = {2005},
note = {A collection of papers presented at the 5th European Conference on Foams, Emulsions, and Applications, EUFOAM 2004, University of Marne-la-Vallee, Champs sur Marne (France), 5-8 July, 2004},
issn = {0927-7757},
doi = {https://doi.org/10.1016/j.colsurfa.2004.10.127},
url = {https://www.sciencedirect.com/science/article/pii/S0927775704008192},
author = {Kenneth Brakke},
keywords = {Soap film, Plateau border, Stability, Cube, Cone},
abstract = {A “dry” conical soap film on a cubical frame is not stable. Recent experimental evidence seems to indicate that adding liquid to form Plateau borders stabilizes the conical film, perhaps to arbitrarily low liquid fractions. This paper presents numerical simulation evidence that the wet cone is unstable for low enough liquid fraction, with the critical liquid fraction being about 0.000278.}
}

@article {BrakkeMorgan,
    AUTHOR = {Brakke, Kenneth and Morgan, Frank},
     TITLE = {Instability of the wet {$X$} soap film},
   JOURNAL = {J. Geom. Anal.},
  FJOURNAL = {The Journal of Geometric Analysis},
    VOLUME = {8},
      YEAR = {1998},
    NUMBER = {5},
     PAGES = {749--767},
      ISSN = {1050-6926},
   MRCLASS = {49Q05 (53A10 76D45)},
  MRNUMBER = {1731061},
MRREVIEWER = {Harold Parks},
       DOI = {10.1007/BF02922669},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/BF02922669},
}

@article {BZ,
    AUTHOR = {Brothers, John E. and Ziemer, William P.},
     TITLE = {Minimal rearrangements of {S}obolev functions},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {384},
      YEAR = {1988},
     PAGES = {153--179},
      ISSN = {0075-4102},
   MRCLASS = {26D10 (26D15 28A75 46E35 49F20)},
  MRNUMBER = {929981},
MRREVIEWER = {Gerald B. Folland},
}

@article{Osgood,
 ISSN = {00029947},
 URL = {http://www.jstor.org/stable/1986455},
 author = {William F. Osgood},
 journal = {Transactions of the American Mathematical Society},
 number = {1},
 pages = {107--112},
 publisher = {American Mathematical Society},
 title = {A Jordan Curve of Positive Area},
 urldate = {2023-09-17},
 volume = {4},
 year = {1903}
}

@article {FangKo,
    AUTHOR = {Fang, Yangqin and Kolasi\'{n}ski, S\l{}awomir},
     TITLE = {Existence of solutions to a general geometric elliptic
              variational problem},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {57},
      YEAR = {2018},
    NUMBER = {3},
     PAGES = {Paper No. 91, 71},
      ISSN = {0944-2669,1432-0835},
   MRCLASS = {49Q20 (28A75 49Q15)},
  MRNUMBER = {3800850},
MRREVIEWER = {Antonio\ Leaci},
       DOI = {10.1007/s00526-018-1348-4},
       URL = {https://doi.org/10.1007/s00526-018-1348-4},
}

@article {Fang,
    AUTHOR = {Fang, Yangqin},
     TITLE = {Existence of minimizers for the {R}eifenberg plateau problem},
   JOURNAL = {Ann. Sc. Norm. Super. Pisa Cl. Sci. (5)},
  FJOURNAL = {Annali della Scuola Normale Superiore di Pisa. Classe di
              Scienze. Serie V},
    VOLUME = {16},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {817--844},
      ISSN = {0391-173X,2036-2145},
   MRCLASS = {49J10 (49Q20)},
  MRNUMBER = {3618078},
MRREVIEWER = {Ilaria\ Fragal\`a},
}

@article {DR,
    AUTHOR = {De Rosa, Antonio},
     TITLE = {Minimization of anisotropic energies in classes of rectifiable
              varifolds},
   JOURNAL = {SIAM J. Math. Anal.},
  FJOURNAL = {SIAM Journal on Mathematical Analysis},
    VOLUME = {50},
      YEAR = {2018},
    NUMBER = {1},
     PAGES = {162--181},
      ISSN = {0036-1410,1095-7154},
   MRCLASS = {49Q20 (49Q15)},
  MRNUMBER = {3742687},
MRREVIEWER = {Panayotis\ Vyridis},
       DOI = {10.1137/17M1112479},
       URL = {https://doi.org/10.1137/17M1112479},
}

@article {DPDRG2,
    AUTHOR = {De Philippis, Guido and De Rosa, Antonio and Ghiraldin,
              Francesco},
     TITLE = {Existence results for minimizers of parametric elliptic
              functionals},
   JOURNAL = {J. Geom. Anal.},
  FJOURNAL = {Journal of Geometric Analysis},
    VOLUME = {30},
      YEAR = {2020},
    NUMBER = {2},
     PAGES = {1450--1465},
      ISSN = {1050-6926,1559-002X},
   MRCLASS = {49Q20 (28A75 49Q15)},
  MRNUMBER = {4081321},
MRREVIEWER = {Salvatore\ Stuvard},
       DOI = {10.1007/s12220-019-00165-8},
       URL = {https://doi.org/10.1007/s12220-019-00165-8},
}

@article {DPDRG,
    AUTHOR = {De Philippis, G. and De Rosa, A. and Ghiraldin, F.},
     TITLE = {A direct approach to {P}lateau's problem in any codimension},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {288},
      YEAR = {2016},
     PAGES = {59--80},
      ISSN = {0001-8708,1090-2082},
   MRCLASS = {49Q20 (28A75 49Q15)},
  MRNUMBER = {3436382},
MRREVIEWER = {S\l awomir\ Kolasi\'{n}ski},
       DOI = {10.1016/j.aim.2015.10.007},
       URL = {https://doi.org/10.1016/j.aim.2015.10.007},
}

@article {CCDPMSteiner,
    AUTHOR = {Cagnetti, Filippo and Colombo, Maria and De Philippis, Guido
              and Maggi, Francesco},
     TITLE = {Rigidity of equality cases in {S}teiner's perimeter
              inequality},
   JOURNAL = {Anal. PDE},
  FJOURNAL = {Analysis \& PDE},
    VOLUME = {7},
      YEAR = {2014},
    NUMBER = {7},
     PAGES = {1535--1593},
      ISSN = {2157-5045},
   MRCLASS = {49K21},
  MRNUMBER = {3293444},
MRREVIEWER = {Sandro Zagatti},
       DOI = {10.2140/apde.2014.7.1535},
       URL = {https://doi.org/10.2140/apde.2014.7.1535},
}
		

@article {CCDPM17,
    AUTHOR = {Cagnetti, Filippo and Colombo, Maria and De Philippis, Guido
              and Maggi, Francesco},
     TITLE = {Essential connectedness and the rigidity problem for
              {G}aussian symmetrization},
   JOURNAL = {J. Eur. Math. Soc. (JEMS)},
  FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
    VOLUME = {19},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {395--439},
      ISSN = {1435-9855},
   MRCLASS = {49Q05 (49K21)},
  MRNUMBER = {3605020},
MRREVIEWER = {Erik J. Balder},
       DOI = {10.4171/JEMS/669},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.4171/JEMS/669},
}

@article {CK,
    AUTHOR = {Cox, Steven J. and Kawohl, Bernhard},
     TITLE = {Circular symmetrization and extremal {R}obin conditions},
   JOURNAL = {Z. Angew. Math. Phys.},
  FJOURNAL = {Zeitschrift f\"{u}r Angewandte Mathematik und Physik. ZAMP.
              Journal of Applied Mathematics and Physics. Journal de
              Math\'{e}matiques et de Physique Appliqu\'{e}es},
    VOLUME = {50},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {301--311},
      ISSN = {0044-2275},
   MRCLASS = {35K05 (35K20)},
  MRNUMBER = {1687057},
MRREVIEWER = {Stepan D. Ivasyshen},
       DOI = {10.1007/s000330050152},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/s000330050152},
}

@article {DGM,
    AUTHOR = {De Lellis, C. and Ghiraldin, F. and Maggi, F.},
     TITLE = {A direct approach to {P}lateau's problem},
   JOURNAL = {J. Eur. Math. Soc. (JEMS)},
  FJOURNAL = {Journal of the European Mathematical Society (JEMS)},
    VOLUME = {19},
      YEAR = {2017},
    NUMBER = {8},
     PAGES = {2219--2240},
      ISSN = {1435-9855},
   MRCLASS = {49Q05 (49Q20)},
  MRNUMBER = {3668059},
MRREVIEWER = {J. Harrison},
       DOI = {10.4171/JEMS/716},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.4171/JEMS/716},
}

@article {DLDRG,
    AUTHOR = {De Lellis, Camillo and De Rosa, Antonio and Ghiraldin,
              Francesco},
     TITLE = {A direct approach to the anisotropic {P}lateau problem},
   JOURNAL = {Adv. Calc. Var.},
  FJOURNAL = {Advances in Calculus of Variations},
    VOLUME = {12},
      YEAR = {2019},
    NUMBER = {2},
     PAGES = {211--223},
      ISSN = {1864-8258},
   MRCLASS = {49Q20 (49Q10)},
  MRNUMBER = {3935858},
MRREVIEWER = {Gwenael Mercier},
       DOI = {10.1515/acv-2016-0057},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1515/acv-2016-0057},
}

@book {F,
    AUTHOR = {Federer, Herbert},
     TITLE = {Geometric measure theory},
    SERIES = {Die Grundlehren der mathematischen Wissenschaften, Band 153},
 PUBLISHER = {Springer-Verlag New York Inc., New York},
      YEAR = {1969},
     PAGES = {xiv+676},
   MRCLASS = {28.80 (26.00)},
  MRNUMBER = {0257325},
MRREVIEWER = {J. E. Brothers},
}

@article {HM,
    AUTHOR = {Hass, Joel and Morgan, Frank},
     TITLE = {Geodesics and soap bubbles in surfaces},
   JOURNAL = {Math. Z.},
  FJOURNAL = {Mathematische Zeitschrift},
    VOLUME = {223},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {185--196},
      ISSN = {0025-5874},
   MRCLASS = {53A10 (49Q20 58E12)},
  MRNUMBER = {1417428},
MRREVIEWER = {Jo\~{a}o Lucas Marques Barbosa},
       DOI = {10.1007/PL00004560},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/PL00004560},
}

@article {HP16,
    AUTHOR = {Harrison, Jenny and Pugh, Harrison},
     TITLE = {Existence and soap film regularity of solutions to {P}lateau's
              problem},
   JOURNAL = {Adv. Calc. Var.},
  FJOURNAL = {Advances in Calculus of Variations},
    VOLUME = {9},
      YEAR = {2016},
    NUMBER = {4},
     PAGES = {357--394},
      ISSN = {1864-8258},
   MRCLASS = {49J45 (46G99 46T30)},
  MRNUMBER = {3552459},
MRREVIEWER = {Martin Fuchs},
       DOI = {10.1515/acv-2015-0023},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1515/acv-2015-0023},
}

@article {HP17,
    AUTHOR = {Harrison, J. and Pugh, H.},
     TITLE = {General methods of elliptic minimization},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {56},
      YEAR = {2017},
    NUMBER = {4},
     PAGES = {Paper No. 123, 25},
      ISSN = {0944-2669},
   MRCLASS = {49Q20 (49J10)},
  MRNUMBER = {3682861},
MRREVIEWER = {Luca Granieri},
       DOI = {10.1007/s00526-017-1217-6},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/s00526-017-1217-6},
}

@article {HT,
    AUTHOR = {Hutchinson, John E. and Tonegawa, Yoshihiro},
     TITLE = {Convergence of phase interfaces in the van der
              {W}aals-{C}ahn-{H}illiard theory},
   JOURNAL = {Calc. Var. Partial Differential Equations},
  FJOURNAL = {Calculus of Variations and Partial Differential Equations},
    VOLUME = {10},
      YEAR = {2000},
    NUMBER = {1},
     PAGES = {49--84},
      ISSN = {0944-2669},
   MRCLASS = {49Q20 (35B25 35B38 35J60 49J45 80A22)},
  MRNUMBER = {1803974},
MRREVIEWER = {Werner Horn},
       DOI = {10.1007/PL00013453},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/PL00013453},
}

@book {K,
    AUTHOR = {Kawohl, Bernhard},
     TITLE = {Rearrangements and convexity of level sets in {PDE}},
    SERIES = {Lecture Notes in Mathematics},
    VOLUME = {1150},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1985},
     PAGES = {iv+136},
      ISBN = {3-540-15693-3},
   MRCLASS = {35-02 (35B50 35J60 49A50)},
  MRNUMBER = {810619},
MRREVIEWER = {Michael Wiegner},
       DOI = {10.1007/BFb0075060},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/BFb0075060},
}

@article {KMS1,
    AUTHOR = {King, Darren and Maggi, Francesco and Stuvard, Salvatore},
     TITLE = {Plateau's problem as a singular limit of capillarity problems
              (revised)},
   JOURNAL = {Comm. Pure Appl. Math.},
  FJOURNAL = {Communications on Pure and Applied Mathematics},
    VOLUME = {75},
      YEAR = {2022},
    NUMBER = {5},
     PAGES = {895--969},
      ISSN = {0010-3640},
   MRCLASS = {53A10 (49Q05)},
  MRNUMBER = {4400904},
MRREVIEWER = {Changwei Xiong},
       DOI = {10.1002/cpa.22048},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1002/cpa.22048},
}

@article {KMS2,
    AUTHOR = {King, Darren and Maggi, Francesco and Stuvard, Salvatore},
     TITLE = {Collapsing and the convex hull property in a soap film
              capillarity model},
   JOURNAL = {Ann. Inst. H. Poincar\'{e} C Anal. Non Lin\'{e}aire},
  FJOURNAL = {Annales de l'Institut Henri Poincar\'{e} C. Analyse Non
              Lin\'{e}aire},
    VOLUME = {38},
      YEAR = {2021},
    NUMBER = {6},
     PAGES = {1929--1941},
      ISSN = {0294-1449,1873-1430},
   MRCLASS = {49Q05 (49Q20 53A10)},
  MRNUMBER = {4327902},
MRREVIEWER = {Chun-Chi\ Lin},
       DOI = {10.1016/j.anihpc.2021.02.005},
       URL = {https://doi.org/10.1016/j.anihpc.2021.02.005},
}

@article {KMS3,
    AUTHOR = {King, Darren and Maggi, Francesco and Stuvard, Salvatore},
     TITLE = {Smoothness of collapsed regions in a capillarity model for
              soap films},
   JOURNAL = {Arch. Ration. Mech. Anal.},
  FJOURNAL = {Archive for Rational Mechanics and Analysis},
    VOLUME = {243},
      YEAR = {2022},
    NUMBER = {2},
     PAGES = {459--500},
      ISSN = {0003-9527,1432-0673},
   MRCLASS = {49Q05 (49Q20)},
  MRNUMBER = {4367906},
MRREVIEWER = {Georgios\ Psaradakis},
       DOI = {10.1007/s00205-021-01727-3},
       URL = {https://doi.org/10.1007/s00205-021-01727-3},
}

@article {KT1,
    AUTHOR = {Kagaya, Takashi and Tonegawa, Yoshihiro},
     TITLE = {A fixed contact angle condition for varifolds},
   JOURNAL = {Hiroshima Math. J.},
  FJOURNAL = {Hiroshima Mathematical Journal},
    VOLUME = {47},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {139--153},
      ISSN = {0018-2079},
   MRCLASS = {49Q15 (28A75)},
  MRNUMBER = {3679887},
MRREVIEWER = {Berardo Ruffini},
       URL = {http://projecteuclid.org.ezproxy.lib.utexas.edu/euclid.hmj/1499392823},
}

@article {KT2,
    AUTHOR = {Kagaya, Takashi and Tonegawa, Yoshihiro},
     TITLE = {A singular perturbation limit of diffused interface energy
              with a fixed contact angle condition},
   JOURNAL = {Indiana Univ. Math. J.},
  FJOURNAL = {Indiana University Mathematics Journal},
    VOLUME = {67},
      YEAR = {2018},
    NUMBER = {4},
     PAGES = {1425--1437},
      ISSN = {0022-2518},
   MRCLASS = {35J20 (35B25 35B38 76D45)},
  MRNUMBER = {3853915},
MRREVIEWER = {Vicen\c{t}iu D. R\u{a}dulescu},
       DOI = {10.1512/iumj.2018.67.7423},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1512/iumj.2018.67.7423},
}

@article {LM,
    AUTHOR = {Leoni, Giovanni and Murray, Ryan},
     TITLE = {Second-order {$\Gamma$}-limit for the {C}ahn-{H}illiard
              functional},
   JOURNAL = {Arch. Ration. Mech. Anal.},
  FJOURNAL = {Archive for Rational Mechanics and Analysis},
    VOLUME = {219},
      YEAR = {2016},
    NUMBER = {3},
     PAGES = {1383--1451},
      ISSN = {0003-9527},
   MRCLASS = {49J45 (35B27 35C20 35J20 49J10)},
  MRNUMBER = {3448931},
MRREVIEWER = {Francesco Maddalena},
       DOI = {10.1007/s00205-015-0924-4},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/s00205-015-0924-4},
}

@article{luckhaus1989gibbs,
  title={The Gibbs-Thompson relation within the gradient theory of phase transitions},
  author={Luckhaus, Stephan and Modica, Luciano},
  journal={Archive for Rational Mechanics and Analysis},
  volume={107},
  number={1},
  pages={71--83},
  year={1989},
  publisher={Springer}
}


@book {maggiBOOK,
    AUTHOR = {Maggi, Francesco},
     TITLE = {Sets of finite perimeter and geometric variational problems},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {135},
      NOTE = {An introduction to geometric measure theory},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2012},
     PAGES = {xx+454},
      ISBN = {978-1-107-02103-7},
   MRCLASS = {49-01 (26B20 28-02 49-02 49Q05 49Q20)},
  MRNUMBER = {2976521},
MRREVIEWER = {Giovanni Alberti},
       DOI = {10.1017/CBO9781139108133},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1017/CBO9781139108133},
}

@misc{MNR1,
      title={Plateau borders in soap films and {G}auss' capillarity theory, ar{X}iv:2310.20169}, 
      author={Francesco Maggi and Michael Novack and Daniel Restrepo},
      year={2023},
      eprint={2310.20169},
      archivePrefix={arXiv},
      primaryClass={math.AP}
}

@misc{MNR2,
      title={A hierarchy of {P}lateau problems and the approximation of {P}lateau's laws via the {A}llen--{C}ahn equation, ar{X}iv:2312.11139}, 
      author={Francesco Maggi and Michael Novack and Daniel Restrepo},
      year={2023},
      eprint={2312.11139},
      archivePrefix={arXiv},
      primaryClass={math.AP}
}

@misc{MR,
  doi = {10.48550/ARXIV.2202.11583},
  
  url = {https://arxiv.org/abs/2202.11583},
  
  author = {Maggi, Francesco and Restrepo, Daniel},
  
  keywords = {Analysis of PDEs (math.AP), Mathematical Physics (math-ph), Optimization and Control (math.OC), FOS: Mathematics, FOS: Mathematics, FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Uniform stability in the {E}uclidean isoperimetric problem for the {A}llen--{C}ahn energy},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@article {MSS,
    AUTHOR = {Maggi, Francesco and Stuvard, Salvatore and Scardicchio,
              Antonello},
     TITLE = {Soap films with gravity and almost-minimal surfaces},
   JOURNAL = {Discrete Contin. Dyn. Syst.},
  FJOURNAL = {Discrete and Continuous Dynamical Systems. Series A},
    VOLUME = {39},
      YEAR = {2019},
    NUMBER = {12},
     PAGES = {6877--6912},
      ISSN = {1078-0947},
   MRCLASS = {49Q05 (49Q15 53A10)},
  MRNUMBER = {4026173},
MRREVIEWER = {Paul Bryan},
       DOI = {10.3934/dcds.2019236},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.3934/dcds.2019236},
}

@article {M,
    AUTHOR = {Modica, Luciano},
     TITLE = {The gradient theory of phase transitions and the minimal
              interface criterion},
   JOURNAL = {Arch. Rational Mech. Anal.},
  FJOURNAL = {Archive for Rational Mechanics and Analysis},
    VOLUME = {98},
      YEAR = {1987},
    NUMBER = {2},
     PAGES = {123--142},
      ISSN = {0003-9527},
   MRCLASS = {76T05 (80A15)},
  MRNUMBER = {866718},
MRREVIEWER = {L. Hsiao},
       DOI = {10.1007/BF00251230},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/BF00251230},
}

@article {MPS,
    AUTHOR = {Morini, Massimiliano and Ponsiglione, Marcello and Spadaro,
              Emanuele},
     TITLE = {Long time behavior of discrete volume preserving mean
              curvature flows},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {784},
      YEAR = {2022},
     PAGES = {27--51},
      ISSN = {0075-4102},
   MRCLASS = {53E10},
  MRNUMBER = {4388339},
MRREVIEWER = {Yue He},
       DOI = {10.1515/crelle-2021-0076},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1515/crelle-2021-0076},
}

@misc{MN23,
      title={Regularity for Minimizers of a Planar Partitioning Problem with Cusps, ar{X}iv:2305.11865}, 
      author={Michael Novack},
      year={2023},
      eprint={2305.11865},
      archivePrefix={arXiv},
      primaryClass={math.AP}
}

@article {Taylor,
    AUTHOR = {Taylor, Jean E.},
     TITLE = {The structure of singularities in soap-bubble-like and
              soap-film-like minimal surfaces},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {103},
      YEAR = {1976},
    NUMBER = {3},
     PAGES = {489--539},
      ISSN = {0003-486X},
   MRCLASS = {49F22 (58A99)},
  MRNUMBER = {428181},
MRREVIEWER = {Klaus Steffen},
       DOI = {10.2307/1970949},
       URL = {https://doi.org/10.2307/1970949},
}


@book {Mil97,
    AUTHOR = {Milnor, John W.},
     TITLE = {Topology from the differentiable viewpoint},
      NOTE = {Based on notes by David W. Weaver},
 PUBLISHER = {University Press of Virginia, Charlottesville, VA},
      YEAR = {1965},
     PAGES = {ix+65},
   MRCLASS = {57.10},
  MRNUMBER = {226651},
MRREVIEWER = {W. S. Piper},
}

@book {Finn,
    AUTHOR = {Finn, Robert},
     TITLE = {Equilibrium capillary surfaces},
    SERIES = {Grundlehren der mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {284},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1986},
     PAGES = {xvi+245},
      ISBN = {0-387-96174-7},
   MRCLASS = {49-02 (49F10 53-02 53A10 58E12)},
  MRNUMBER = {816345},
MRREVIEWER = {Helmut Kaul},
       DOI = {10.1007/978-1-4613-8584-4},
       URL = {https://doi.org/10.1007/978-1-4613-8584-4},
}

@book {Simon,
    AUTHOR = {Simon, Leon},
     TITLE = {Lectures on geometric measure theory},
    SERIES = {Proceedings of the Centre for Mathematical Analysis,
              Australian National University},
    VOLUME = {3},
 PUBLISHER = {Australian National University, Centre for Mathematical
              Analysis, Canberra},
      YEAR = {1983},
     PAGES = {vii+272},
      ISBN = {0-86784-429-9},
   MRCLASS = {49-01 (28A75 49F20)},
  MRNUMBER = {756417},
MRREVIEWER = {J. S. Joel},
}

@article {S,
    AUTHOR = {Sternberg, Peter},
     TITLE = {The effect of a singular perturbation on nonconvex variational
              problems},
   JOURNAL = {Arch. Rational Mech. Anal.},
  FJOURNAL = {Archive for Rational Mechanics and Analysis},
    VOLUME = {101},
      YEAR = {1988},
    NUMBER = {3},
     PAGES = {209--260},
      ISSN = {0003-9527},
   MRCLASS = {49A50 (49F10 76A02)},
  MRNUMBER = {930124},
MRREVIEWER = {Luciano Modica},
       DOI = {10.1007/BF00253122},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/BF00253122},
}

@article {TW,
    AUTHOR = {Tonegawa, Yoshihiro and Wickramasekera, Neshan},
     TITLE = {Stable phase interfaces in the van der
              {W}aals--{C}ahn--{H}illiard theory},
   JOURNAL = {J. Reine Angew. Math.},
  FJOURNAL = {Journal f\"{u}r die Reine und Angewandte Mathematik. [Crelle's
              Journal]},
    VOLUME = {668},
      YEAR = {2012},
     PAGES = {191--210},
      ISSN = {0075-4102},
   MRCLASS = {58E50 (35B25 35J20 49Q05)},
  MRNUMBER = {2948876},
MRREVIEWER = {Futoshi Takahashi},
       DOI = {10.1515/crelle.2011.134},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1515/crelle.2011.134},
}

@article {V,
    AUTHOR = {Villa, Elena},
     TITLE = {On the outer {M}inkowski content of sets},
   JOURNAL = {Ann. Mat. Pura Appl. (4)},
  FJOURNAL = {Annali di Matematica Pura ed Applicata. Series IV},
    VOLUME = {188},
      YEAR = {2009},
    NUMBER = {4},
     PAGES = {619--630},
      ISSN = {0373-3114},
   MRCLASS = {28A75 (49Q15)},
  MRNUMBER = {2533959},
MRREVIEWER = {Hany M. Farag},
       DOI = {10.1007/s10231-008-0093-2},
       URL = {https://doi-org.ezproxy.lib.utexas.edu/10.1007/s10231-008-0093-2},
}

@book{foamchapter,
    author = {Cantat, I. and Cohen-Addad, S. and Elias, F. and Graner, F. and H\"{o}hler, R. and
     Pitois, O. and Rouyer, F. and Saint-Jalmes, A. and Flatman, R. and Cox, S.},
    title = {Foams: {S}tructure and {D}ynamics},
    publisher = {Oxford University Press},
    year = {2013}}

@book{weaireBOOK,
author={Weaire, D. and Hutzler, S.},
title={The Physics of Foams},
year={1999},
publisher={Oxford University Press}
}
